Secure Computation with Shared EPR Pairs (Or: How to Teleport in Zero-Knowledge)

Can a sender non-interactively transmit one of two strings to a receiver without knowing which string was received? Does there exist minimally-interactive secure multiparty computation that only makes (black-box) use of symmetric-key primitives? We provide affirmative answers to these questions in a model where parties have access to shared EPR pairs, thus demonstrating the cryptographic power of this resource. First, we construct a one-shot (i.e., single message) string oblivious transfer (OT) protocol with random receiver bit in the shared EPR pairs model, assuming the (sub-exponential) hardness of LWE. Building on this, we show that {\em secure teleportation through quantum channels} is possible. Specifically, given the description of any quantum operation $Q$, a sender with (quantum) input $\rho$ can send a single classical message that securely transmits $Q(\rho)$ to a receiver. That is, we realize an ideal quantum channel that takes input $\rho$ from the sender and provably delivers $Q(\rho)$ to the receiver without revealing any other information. This immediately gives a number of applications in the shared EPR pairs model: (1) non-interactive secure computation of unidirectional \emph{classical} randomized functionalities, (2) NIZK for QMA from standard (sub-exponential) hardness assumptions, and (3) a non-interactive \emph{zero-knowledge} state synthesis protocol. Next, we construct a two-round (round-optimal) secure multiparty computation protocol for classical functionalities in the shared EPR pairs model that is \emph{unconditionally-secure} in the (quantum-accessible) random oracle model.

==> impossibility.tex <==
\section{Impossibility of One-Shot OT in the CRS Model}

\begin{theorem}
There does not exist a one-message protocol that securely realizes (\cref{def:secure-realization}) the functionality $\cF_\ROT$ in the common reference string model.
\end{theorem}

\begin{proof}
We will use the following imported theorem, which is a special case of \cite[Claim 3.5]{cryptoeprint:2022/786}.

\begin{importedtheorem}[\cite{cryptoeprint:2022/786}]\label{impthm:DS}
Let $\sD$ be a projector, $\Pi_0,\Pi_1$ be orthogonal projectors, and $\ket{\psi} \in \mathsf{Im}\left(\Pi_0+\Pi_1\right)$. Then,

\[\|\Pi_1\sD\Pi_0\ket{\psi}\|^2 + \|\Pi_0\sD\Pi_1\ket{\psi}\|^2 \geq \frac{1}{2}\left(\|\sD\ket{\psi}\|^2 - \left(\|\sD\Pi_0\ket{\psi}\|^2 + \|\sD\Pi_1\ket{\psi}\|^2 \right)\right)^2.\]
\end{importedtheorem}

Now consider any one-message protocol for $\cF_\ROT$, where the common reference string is sampled as $\crs \gets \cR$ from some distribution $\cR$ over classical strings. Fix any pair of sender inputs $(m_0,m_1)$, and let $\ket{\psi}$ be the message sent by the honest sender on input $m_0,m_1$ and $\crs$ (note that $\ket{\psi}$ is a sample from a distribution). Without loss of generality, we can consider the honest receiver strategy to apply a unitary $U_R$ on $\ket{\psi}\ket{0}$ (where the auxiliary register is initialized with sufficiently many qubits) and then measure an output register in the standard basis to obtain $(b,m_b)$. We define

\[\Pi_0 \coloneqq U_R^\dagger\dyad{0,m_0}{0,m_0}U_R, \ \ \, \Pi_1 \coloneqq U_R^\dagger\dyad{1,m_1}{1,m_1}U_R.\] 

Suppose that the protocol satisfies perfect correctness.\footnote{If it satisfies $1-\negl(\secp)$ correctness, our arguments will be valid up to $\negl(\secp)$ loss, by Gentle Measurement.} It follows that $\ket{\psi} \in \mathsf{Im}(\Pi_0 + \Pi_1)$. Now, suppose that an adversarial sender applies the measurement $\{\Pi_0,\Pi_1\}$ to $\ket{\psi}$ and then sends the resulting mixture over $\Pi_0\ket{\psi}$ and $\Pi_1\ket{\psi}$ to the receiver. There are two cases.

In the first case, there does not exist a QPT procedure that distinguishes $\ket{\psi}$ from the mixture over $\Pi_0\ket{\psi}$ and $\Pi_1\ket{\psi}$. In this case, the sender learns the bit $b$ obtained by the receiver from the outcome of measurement $\{\Pi_0,\Pi_1\}$, which violates security.

In the second case, there exists a QPT distinguisher $\sD$ (written as a projective measurement) that distinguishes with $\nonnegl(\secp)$ probability. Then by \cref{impthm:DS}, we have that \[\E_{\crs,\ket{\psi}}\left[\|\Pi_1\sD\Pi_0\ket{\psi}\|^2 + \|\Pi_0\sD\Pi_1\ket{\psi}\|^2\right] = \nonnegl(\secp),\] where the expectation is over the sampling of $\crs \gets \cR$ and the sampling of the sender's message $\ket{\psi}$. However, this means that the following receiver strategy will return $\{m_0,m_1\}$ with $\nonnegl(\secp)$ probability, which violates security. Begin with $\ket{\psi}\ket{0}$. Apply $U_R$ and measure the output register in the computational basis to obtain $(b,m_b)$. Then, apply $U_R \sD U_R^\dagger$ and measure the output register in the computational basis to obtain $(1-b,m_{1-b})$. This completes the proof.

\end{proof}
